Infinite loop spaces associated to affine Kac-Moody groups

It is well known that to each infinite class of classical groups over a commutative ring $R$, we can associate an infinite loop space by Quillen's plus construction. In this paper we generalize this fact to the case of affine Kac-Moody groups.

==> 0230113.tex <==
%auto-ignore
